Inferring and predicting Fried physical frailty phenotype deficits

We predict the Fried physical frailty phenotype health deficits (FPFP5: slow gait, weakness, weight loss, low activity, and exhaustion) using two measures of frailty: frailty index (FI) or frailty phenotype (FP). The FP theorizes that the FPFP5 are mutually dependent through shared etiology and positive feedbacks, so that the total number of FPFP5 deficits (NFPFP5) should be highly predictive of existing deficits. Alternatively, the FI theorizes that strong mutual dependencies exist between \emph{all} age-related health deficits, so that the FI would be more predictive. We investigated predictive models of FPFP5 using FI or NFPFP5 in the Health and Retirement Study (HRS), the English Longitudinal Study of Aging (ELSA), and the National Health and Nutrition Examination Survey (NHANES). We find that the FI, chronological age, and current deficit state are all important predictors of future FPFP5 deficits. Notably, the FI consistently out-performed NFPFP5, raising questions regarding FPFP5 causal connections and how best to measure the physical component of frailty. We discuss implications for both FPFP5 forecasting, and inference when data are missing or incomplete.

==> PREVIOUS/cutouts.tex <==
\section{Results}

\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/age.pdf} 
        \caption{Age-related changes. The FI is increasing super-linearly with age (red line) whereas the FP does not show a clear age-related trend (blue line).}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ttd.pdf} 
        \caption{Terminal decline. The FI increases as death becomes increasingly imminent (red line) whereas the FP does not show a clear change (blue line). Note the much larger uncertainty in the FP (blue) vs FI (red).}
    \end{subfigure}
    \caption{Changes to FI and FP with age and time-to-death. The FI (red) is clearly more sensitive to age and health--related changes than the FP (blue). Also note the larger uncertainty (dispersion) in the FP versus the FI, which could reflect a lack of resolution. All individuals were followed for at least 12.9 years. After 12.9 years the censored and dead individuals showed identical trends (Supplemental).} \label{fig:demo}
\end{figure*}


%%%%%%%%%%
\begin{figure*}[!ht] %don't allow page floats
     \centering
        \includegraphics[width=\textwidth]{figures/auc.pdf}  
    \caption{Predictive power for predicting the key FP biomarkers (AUC). Higher is better: 0.5 is a guess, 1 is perfect. FI: total frailty index (lab and clinical). FP variables: the 4 complementary FP biomarker values used to predict the 5th. Number of FP deficits: average number of FP deficits, excluding the predicted. The FI and the FI CLINIC are better able to predict FP deficits than the other FP biomarkers.}
    \label{fig:auc}
\end{figure*}


\begin{figure*}[!ht] %don't allow page floats
     \centering
        \includegraphics[width=0.5\textwidth]{figures/roc.pdf}  
    \caption{Predictive power for predicting FP using the FI. AUC: 0.87 (0.80-0.95, 95\% CI).}
    \label{fig:roc}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/fp_vs_fi.pdf}
    \caption{FP vs FI. We see a clear threshold effect in the FP score, where it is insensitive to small changes in the FI.} \label{fig:fp_vs_fi}
\end{figure}


\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|}
    \hline
         & FI $\leq$ 0.21 & FI > 0.21 \\ \hline
        Robust & & \\ \hline
        Pre-frail & & \\ \hline
        Frail & & \\ \hline
    \end{tabular}
    \caption{\label{tab:fp_vs_fi} FP vs FI.}
\end{table}


\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ttd_models.pdf} 
        \caption{Spline models for terminal decline. GAM, spline with 5 knots. FP appears to have a threshold whereas FI does not. Note the much larger uncertainty in the FP (blue) vs FI (red). Notice that FI crosses $0$ before $1$ (Arnold estimated death was certain at 0.45, upper limit 0.55 (95\% CI)\cite{Mitnitski2006-fq})}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/hr.pdf} 
        \caption{Log--hazard rates/ratios of the FP and FI (Cox coefficient, $\beta$). x-axis is the FP on its native scale (number of deficits); we have scaled the FI to the same range as the FP. FI appears to be linear, whereas FP seems to have a threshold. Points: Cox model using ordinal scales (deciles for FI). Lines are Cox models treating FI and FP as continuous predictors. Notice that the FI line fits the FP points better than the FI line.}
    \end{subfigure}
    \caption{Survival modelling suggests that the FP has a threshold, where-in an increase from 1 to 2 shows no change in survival risk. In contrast, the FI shows a monotonic, linear, increase in risk. If the FI is scaled to the range of the FP (b), it appears to interpolate the FP risk: since the last FI point is 0.38.} \label{fig:surv}
\end{figure*}
